Computational dynamics of acoustically-driven microsphere systems

We propose a computational framework for the self-consistent dynamics of a microsphere system driven by a pulsed acoustic field in an ideal fluid. Our framework combines a molecular dynamics integrator describing the dynamics of the microsphere system with a time-dependent integral equation solver for the acoustic field that makes use of fields represented as surface expansions in spherical harmonic basis functions. The presented approach allows us to describe the inter-particle interaction induced by the field as well as the dynamics of trapping in counter-propagating acoustic pulses. The integral equation formulation leads to equations of motion for the microspheres describing the effect of non-dissipative drag forces. We show (1) that the field-induced interactions between the microspheres give rise to effective dipolar interactions, with effective dipoles defined by their velocities, and (2) that the dominant effect of an ultrasound pulse through a cloud of microspheres gives rise mainly to a translation of the system, though we also observe both expansion and contraction of the cloud determined by the initial system geometry.

==> figures/banding_peakAcc_vs_displacement.tex <==
\begin{tikzpicture}
  \begin{axis}[
    xlabel = {Displacement $(\si{\meter})$},
    ylabel = {Peak acceleration $(\si{\meter \per \second^2})$},
    grid = major
  ]
    \addplot[
      coolblue,
      only marks
    ] table {data/bluegroup.dat};

    \addplot[
      warmred,
      only marks
    ] table {data/redgroup.dat};
  \end{axis}
\end{tikzpicture}


==> figures/single_particle_displacement.tex <==
\begin{tikzpicture}
  \begin{axis}[
    xlabel={Time $(\si{\micro\second})$},
    ylabel={Displacement $(\si{\micro\meter})$},
    grid=major,
    cycle multi list = {Set1-3}, 
  ]
    \addplot+[
      black, solid, smooth, thick
    ] table [
    ] {data/single_bubble_sigmoid.dat};

  \end{axis}
\end{tikzpicture}

